Femtosecond X-ray Fourier holography imaging of free-flying nanoparticles

Ultrafast X-ray imaging provides high resolution information on individual fragile specimens such as aerosols, metastable particles, superfluid quantum systems and live biospecimen, which is inaccessible with conventional imaging techniques. Coherent X-ray diffractive imaging, however, suffers from intrinsic loss of phase, and therefore structure recovery is often complicated and not always uniquely-defined. Here, we introduce the method of in-flight holography, where we use nanoclusters as reference X-ray scatterers in order to encode relative phase information into diffraction patterns of a virus. The resulting hologram contains an unambiguous three-dimensional map of a virus and two nanoclusters with the highest lat- eral resolution so far achieved via single shot X-ray holography. Our approach unlocks the benefits of holography for ultrafast X-ray imaging of nanoscale, non-periodic systems and paves the way to direct observation of complex electron dynamics down to the attosecond time scale.

==> packages.tex <==
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[ngerman]{babel}
\usepackage{paralist}
\usepackage{array}
\usepackage{mathrsfs,amsmath}
\usepackage{amssymb}
\usepackage{dsfont}
\usepackage{ragged2e}
\usepackage{fancyhdr}
\usepackage{booktabs}
\usepackage{url}
\usepackage{bbm}
%\usepackage{xcolor}
\usepackage[a4paper, includeheadfoot, top=22mm, bottom=20mm, textheight=240mm, footskip=20mm,left=30mm,right=20mm]{geometry}
% Brunos:
% \usepackage[textwidth=145mm,textheight=235mm,left=35mm,top=30mm,headsep=10mm]{geometry}
\usepackage{titlesec}
\usepackage[margin=10pt, font=small, labelfont=bf, skip= 5pt]{caption}
\usepackage{multirow}
\usepackage{comment}
\usepackage{overpic}
\usepackage{subfig}
\usepackage{placeins}
\usepackage{epstopdf}
\usepackage{epigraph}
\usepackage[framed,numbered,autolinebreaks,useliterate]{mcode}
\usepackage{appendix} %um eine Titelseite "Anhang" vor dem eigentlichen Anhang einfügen zu können
\usepackage{overpic}
%\usepackage[round]{natbib}
\usepackage[numbers,sort&compress]{natbib}
\usepackage[decimalsymbol=comma,separate-uncertainty,range-phrase=--,range-units=single]{siunitx}
%\usepackage{mathtools}
\usepackage{lscape}
\usepackage{import}
\usepackage{color} 
\usepackage{transparent}
\usepackage{layouts}
\usepackage{floatflt} 
\usepackage{graphicx}
\usepackage{bm}

\usepackage{hyperref} %pdf-Inhaltsverzeichnis und pdf-Links
\hypersetup{
	pdfborder={0 0 0}, 
	bookmarksnumbered=true,
	pdftitle={Untersuchung von Röntgen-Streubildern einzelner Nanopartikel -- Neue Ansätze zur Lösung des Phasenproblems},
	pdfauthor={Anatoli Ulmer}
}

%Druckt den Hinweis "Entwurf" mit Datum auf jede Seite. Zum deaktivieren printwatermark=false setzen
%\usepackage[printwatermark=true]{xwatermark}
%\newwatermark[allpages,textcolor=gray!70,angle=0,xpos=68,ypos=-135,fontsize=14pt,fontfamily=phv]{Entwurf\ -\ \the\day.\the\month.\the\year}

%Appendices -> Anhang
\renewcommand*\appendixpagename{Anhang}
\renewcommand*\appendixtocname{Anhang}

\pagestyle{fancy}
\fancyhf{}
\fancyhead[LO]{\sc\nouppercase\rightmark} 
\fancyhead[RE]{\sc\nouppercase\leftmark}
%\lhead{}%\leftmark}
%\rhead{\leftmark}
%\fancyfoot[LE,RO]{\thepage}
\cfoot{\thepage}

%\renewcommand{\sectionmark}[1]{% 
%	\markboth{\thesection.\ #1}{}}

\newcommand{\red}[1]{\textcolor{red}{#1}}

\titleformat{\section}
{\normalfont\LARGE\bfseries}{\thesection}{1em}{}
\titleformat{\subsection}
{\normalfont\Large\bfseries}{\thesubsection}{1em}{}
\titleformat{\subsubsection}
{\normalfont\large\bfseries}{\thesubsubsection}{1em}{}
\titleformat{\paragraph}[hang]
{\normalfont\normalsize\bfseries}{\theparagraph}{1em}{}

\setlength{\textfloatsep}{10pt}
\setlength{\parindent}{0ex}
\setlength{\parskip}{1ex}

%\numberwithin{equation}{section}

%\newcommand{\sectionbreak}{%
%	\clearpage%
%	\newpage%
%	\addpenalty{-300}
%	\vspace*{0pt}}

\newcommand{\bra}[1]{\langle #1|}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\braket}[2]{\langle #1|#2 \rangle}
\newcommand{\av}[1]{\langle #1 \rangle}

\newcommand{\tr}[1]{\mbox{Tr}\left(#1 \right)}
\newcommand{\re}[1]{\mbox{Re}\left(#1 \right)}
\newcommand{\im}[1]{\mbox{Im}\left(#1 \right)}
\newcommand{\entspricht}{\mathrel{\widehat{=}}}
\newcommand{\abs}[1]{\lvert #1 \rvert}

\newcommand*{\mathcolor}{}
\def\mathcolor#1#{\mathcoloraux{#1}}
\newcommand*{\mathcoloraux}[3]{%
	\protect\leavevmode
	\begingroup
	\color#1{#2}#3%
	\endgroup
}

\definecolor{azure}{rgb}{0.0, 0.5, 1.0}

\newcommand{\myincludegraphics}[3][\linewidth]{%
		\def\svgwidth{#1}%
		\import{#2}{#3}%
}

\newcommand{\FF}{\mathscr{F}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\z}[1]{\SI{#1}{}}


\usepackage{lmodern}

\newcommand*\Hide{%
	\titleformat{\chapter}[display]
	{}{}{0pt}{\Huge}
	\titleformat{\part}
	{}{}{0pt}{}
}

